Centralized Versus Distributed Routing for Large-Scale Satellite Networks

An important choice in the design of satellite networks is whether the routing decisions are made in a distributed manner onboard the satellite, or centrally on a ground-based controller. We study the tradeoff between centralized and distributed routing in large-scale satellite networks. In particular, we consider a centralized routing scheme that has access to global but delayed network state information and a distributed routing scheme that has access to local but real-time network state information. For both routing schemes, we analyze the throughput and delay performance of shortest-path algorithms in networks with and without buffers onboard the satellites. We show that distributed routing outperforms centralized routing when the rate of changes in the network link state is comparable to the inherent propagation and transmission delays. In particular, we show that in highly dynamic networks without buffers, the distributed scheme achieves higher throughput than a centralized scheme. In networks with buffers, the distributed scheme achieves lower delays with the same throughput.

==> WRONG.tex <==
The proof of Lemma \ref{lemma:ordering} entails solving another dynamic program, as described in \cite[Section 4]{akrida_how_2020_journal}. 
Let us assume we have an ordering of vertices in the network $L \triangleq \{(u_1,v_1), (u_2, v_2), ...\}$ such that for $i < j$, $\bar D(u_i, v_i) \leq \bar D(u_j, v_j)$. Note that it suffices to only keep vertices for which $0 \leq u \leq v \leq \lfloor \frac{N}{2}\rfloor$ in the list, as from the symmetry of the network, $\bar D(u,v) = \bar D(v,u) = \bar D(-u, v) = \bar D(u, -v)$. 

Once we have an ordering, we note that when we are at node $(u_j, v_j)$, we move to the next node, say $(u_i, v_i)$, only if all the following conditions are satisfied:
\begin{enumerate}
    \item The link from $(u_j,v_j)$ to $(u_i,v_i)$ is ON
    \item $(u_i,v_i)$ appears in the ordering before $(u_j,v_j)$ (i.e., $i < j$), and
    \item For all $k < i$, the link from $(u_j,v_j)$ to $(u_k,v_k)$ is OFF or does not exist.
\end{enumerate}
If any of the conditions are not satisfied, we wait at $(u_j,v_j)$ as there is no advantage in moving to another node which appears after $(u_j,v_j)$ in the ordering. This translates to the mean delays satisfying the following Bellman equation. 
\begin{equation}
\begin{aligned}
    \bar D(u_j,v_j) &= 1 + \sum_{i=1}^{j-1} p_{u_j,v_j}^{u_i,v_i} \prod_{k=1}^{i-1}(1 - p_{u_j,v_j}^{u_k,v_k})\bar D(u_i, v_i)\\
    &\qquad+ \prod_{i=1}^{j-1}(1 - p_{u_j,v_j}^{u_i,v_i}) \bar D(u_j, v_j),
\end{aligned}
\end{equation}
where $p_{u_j,v_j}^{u_i,v_i}$ denotes the probability of there exists a link between $(u_j, v_j)$ to $(u_i, v_i)$.
In other words, for all $0 \leq j \leq |L|$,
\begin{equation}
\begin{aligned}
    \bar D(u_j,v_j) &= \frac{1 + \sum_{i=1}^{j-1} p_{u_j,v_j}^{u_i,v_i} \prod_{k=1}^{i-1}(1 - p_{u_j,v_j}^{u_k,v_k})\bar D(u_i, v_i)}{ 1 -\prod_{i=1}^{j-1}(1 - p_{u_j,v_j}^{u_i,v_i}) }.
\end{aligned}
\end{equation}
To construct the ordered list $L$, we use a bottom-up approach (as described in \cite[Algorithm 4]{akrida_how_2020_journal}). Observe that Algorithm \ref{algo:ordering} would populate nodes $(u,v)$ into $L$ in order of their mean delay. In Algorithm \ref{algo:ordering}, we use the definition
\begin{equation}\label{eqn:h_def}
    h(u,v,t) \triangleq \frac{1 + \sum_{i=1}^{t} p_{u,v}^{u_i,v_i} \prod_{k=1}^{i-1}(1 - p_{u,v}^{u_k,v_k})\bar D(u_i, v_i)}{ 1 -\prod_{i=1}^{t}(1 - p_{u,v}^{u_i,v_i}) },
\end{equation}
where $(u_i, v_i)$ are the $i^{th}$ nodes in the ordering $L$.
\begin{algorithm}[!hbt]
\caption{Ordering Mean Delays $\bar D(u,v)$} \label{algo:ordering}
    \begin{algorithmic}[1]
        \STATE $L \gets \{(0,0)\}, \bar D(0,0) = 0$.
        \FOR {iteration $t \in \left\{ 1, ..., \frac{1}{2}\lfloor\frac{N}{2}\rfloor(\lfloor\frac{N}{2}\rfloor - 1) \right\}$}
            \STATE $L' \gets \{ (u,v) \notin L, 0\leq u \leq v\leq \lfloor\frac{N}{2}\rfloor \} $ 
            \STATE 
            $(u_{t+1}, v_{t+1}) \gets
                    \argmin_{(u,v) \in L'} h (u,v,t)$ \COMMENT{ As in \eqref{eqn:h_def}}

            \STATE $\bar D (u_{t+1}, v_{t+1}) \gets h(u_{t+1}, v_{t+1}, t)$ \COMMENT{ As in \eqref{eqn:h_def}}

            \STATE Append $(u_{t+1}, v_{t+1}) $ to $L$.
            
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

We are finally equipped to prove Lemma \ref{lemma:ordering}. Consider the following induction hypothesis: in every iteration $t$ of Algorithm \ref{algo:ordering}, $u_{t+1} + v_{t+1} > u_t + v_t$, or, $u_{t+1} + v_{t+1} = u_t + v_t$ and $v_{t} - u_{t} < v_{t+1} - u_{t+1}$.

==> deterministic_greedy.tex <==
Consider a variant of the greedy routing policy wherein, if both the vertical link $l_v$ and horizontal link $l_h$ that take us closer to the destination are ON, we move in the direction along which we are farther from destination. In other words, if we are at node $(x,y)$ and both outgoing links are ON, we move along the vertical if $y>x$ and move along the horizontal if $x > y$. If $x=y$, we break the tie by a fair coin toss. 

This method of breaking ties ensures that we stay \textbf{as close to the diagonal as possible} while routing the packet through the grid network. 
% For the sake of brevity, we do not analytically analyze such a policy. Using numerical results, we can see that the deterministic variant of the GR Policy is better than the randomized version of the GR policy. 
It also turns out that this policy is the \textit{optimal} distributed routing algorithm when the network links have no memory, i.e., $\mu = 0$. When there is no memory $(\mu = 0)$ in the system, equations in \eqref{eqn:transition_k} are equal to the steady state probability. In other words
\begin{equation*}
    \begin{aligned}
        p_{00}(k) &= p_{10}(k) = 1-p \\
        p_{01}(k) &= p_{11}(k) = p 
    \end{aligned} \qquad \forall k,
\end{equation*}
which means that for any $t' \neq t$, knowing the link state $l(t')$ gives you no new information about the link state $l(t)$. This in turn suggests that the optimal policy would only depend the knowledge of the state of the outgoing link at the current node $(x, y)$, the steady state probability $p$ and the logical topology of the network.


\subsection{Optimal Distributed Routing Policy for Mean Delay with Onboard Buffering}

Let $D^*(x,y, l_l, l_d, l_r, l_u)$ denote the minimum mean delay from node $(x,y)$ to $(0,0)$ conditioned on the current states of the outgoing links at $(x,y)$, captured by $l_l, l_d, l_r, l_u$.
The state of the down link is denoted by $l_d$, state of the left link is denoted by $l_l$, state of the up link is denoted by $l_u$, and  state of the right link is denoted by $l_r$. 
Clearly, $l_l, l_d, l_r, l_u \in \{0,1\}$ denoting the ON/OFF state of the link.

From the symmetry of the network, we require
\begin{equation}
    \begin{aligned}
        D^*(x,y,l_l, l_d, l_r, l_u) &= D^*(-x,y,l_r, l_d, l_l, l_u)\\
        &= D^*(x,-y,l_l, l_u, l_r, l_d)\\
        &= D^*(y,x,l_d, l_l, l_u, l_r),
    \end{aligned}
\end{equation}
and so it suffices to study the case when $y \geq x \geq 0$ without loss of generality.

Since $D^*(x,y,l_l, l_d, l_r, l_u)$ is the minimum mean delay, it satisfies the following Bellman equation
\begin{equation}
    D^*(x,y,l_l, l_d, l_r, l_u) = 1 + \min_{(a_x,a_y) \in \mathcal{A}(l_l, l_d, l_r, l_u)} \bar D(x+a_x, y+a_y).\label{eqn:bellman_delay}
\end{equation}

In equation \eqref{eqn:bellman_delay}, $\bar D(x,y)$ is the unconditional minimum mean delay from $(x,y)$ to $(0,0)$. In other words,
\begin{equation}
    \begin{aligned}
        &\bar D(x,y) \\
        &= \sum_{(l'_l, l'_d, l'_r, l'_u) \in \{0,1\}^4} D^*(x,y,l'_l, l'_d, l'_r, l'_u)\cdot P(l'_l, l'_d, l'_r, l'_u),
    \end{aligned}
\end{equation}
where $P(l'_l, l'_d, l'_r, l'_u)$ denotes the probability of the outgoing links having state $l'_l,l'_d,l'_r$ and $l'_u$. It is easy to see that $$
P(l'_l, l'_d, l'_r, l'_u) = p^{l'_l+l'_d+l'_r+l'_u} \times (1-p)^{4 - (l'_l+l'_d+l'_r+l'_u)}.
$$
Additionally, in equation \eqref{eqn:bellman_delay}, $\mathcal{A}(l_l, l_d, l_r, l_u)$ denotes the set of allowable actions conditioned on the state of the outgoing links. In other words,
$$\mathcal{A}(l_l, l_d, l_r, l_u) \subseteq \{(0,0), (-1,0), (0,-1), (1,0), (0,1)\},$$
where $(0,0)$ corresponds to buffering at the current node, $(-1,0)$ corresponds to forwarding the packet along the left link, $(0,-1)$ corresponds to forwarding the packet along the down link, $(1, 0)$ corresponds to forwarding the packet along the right link and $(0,1)$ corresponds to forwarding the packet along the up link, and  $\mathcal{A}(l_l, l_d, l_r, l_u)$ only contains the actions that are permitted by the current link states.

Consequently, the optimal action at a node is to send the packet to the next node which minimizes the unconditional mean delay, as long as it is permitted. In other words, if the packet is at node $(x,y)$, it is only advantageous to forward the packet to its neighbor $(u,v)$ if $\bar D(u,v) < \bar D(x,y)$. If that is not the case, we buffer the packet. In order to find the minimum unconditional mean delay, we need a way to order $\bar D(u,v)$ for every node $(u,v)$ in the satellite network. The way to do this is described in Lemma \ref{lemma:ordering}, whose proof is provided in Appendix \ref{appendix:proof_of_ordering_lemma}.

\begin{lemma}[Mean Delay Ordering of Nodes]\label{lemma:ordering}
For two nodes $(u_1, v_1)$ and $(u_2, v_2)$,
\begin{align}
    \bar D(u_1,v_1) < \bar D(u_2, v_2)
\end{align}
if $|u_1| + |v_1| < |u_2| + |v_2|$, or, $|u_1| + |v_1| = |u_2| + |v_2|$ and $||u_1| - |v_1|| < ||u_2| - |v_2||$.
\end{lemma}

Now, at node $(x,y)$, ($y \geq x \geq 0$ w.l.o.g.), we observe that regardless of the current link states, we would never forward the packet along the up link or right link as $\bar D(x,y) < \bar D(x+1, y)$ and $\bar D(x,y) < \bar D(x, y+1)$ from Lemma \ref{lemma:ordering}. If $x = 0$, then we would never forward the packet further to the left as $\bar D(0,y) < \bar D(-1,y) = \bar D(1, y)$, again from Lemma \ref{lemma:ordering}. Furthermore, observe that in the following cases, when $y \geq x > 0$:
\begin{enumerate}[wide, labelindent=0pt]
    \item \underline{Left link is OFF and down Link is OFF}: As described above, we would not forward along the up and right link, and so the optimal action is to buffer the packet at $(x,y)$.
    \item \underline{Left link is ON and down Link is OFF}: As $\bar D(x-1, y) < \bar D(x,y)$, we forward along the left link.
    \item \underline{Left link is OFF and down Link is ON}: As $\bar D(x, y-1) < \bar D(x,y)$, we forward along the down link.
    \item \underline{Left link and Down Link are both ON}: As $\bar D(x, y-1) < \bar D(x,y)$ and $\bar D(x-1, y) < \bar D(x,y)$, we need to choose where to forward the packet. Since $y \geq x$, note that $|(y - 1) - x| < |y - (x-1)|$, and hence $\bar D(x,y-1) < \bar D(x-1,y)$ from Lemma \ref{lemma:ordering}. Therefore, we would choose to forward along the down link, which is the dimension along which we are further away from the destination.
\end{enumerate}

Hence, the deterministic variant of the greedy algorithm is mean delay optimal with onboard buffering when $\mu = 0$.

\subsection{Optimal Distributed Routing Policy for Throughput without Onboard Buffering}
Similar to the previous subsection, let $h^*(x,y, l_l, l_d, l_r, l_u)$ denote the negative log probability of reaching the destination $(0,0)$ from node $(x,y)$ conditioned on the current states of the outgoing links at $(x,y)$, captured by $l_l, l_d, l_r, l_u$.


==> lemma1_proof.tex <==
The proof is quite straightforward. For connected paths, 
$$\prod_{i=0}^{|\pi|-1} \P(l^\pi_i(t_c + i) = 1 | \b{l}(0)) = \prod_{i=0}^{|\pi|-1}p_{11}(t_c + i).$$
Therefore, 
$$|\pi| \leq |\pi'| \Leftrightarrow \prod_{i=0}^{|\pi|-1}p_{11}(t_c + i) \geq \prod_{i=0}^{|\pi'|-1}p_{11}(t_c + i).$$

==> optimality.tex <==
\section{Optimal Policies}\label{sec:optimality}
\color{red}
I am thinking of skipping this section due to the lack of space.
\color{black}
\subsection{Optimal Centralized Policy In Scenario A}\label{sec:centralized_optimality_scenA}
We want the router to produce a path that maximizes the probability that the packet reaches the destination successfully after some time using the network state information at $t = 0$. The probability of successfully reaching the destination is the probability that every link along the specific path is ON to be traversed. So, in other words, the router needs to solve the following optimization problem
\begin{equation}
    \begin{aligned}
    \min_{\pi \in \Pi} \quad & \prod_{i=0}^{|\pi|-1} \P\bigg(l^\pi_i(t_c + i) = 1 \bigg| \b{l}(0)\bigg).
    \end{aligned}\label{eqn:centralized_scenarioA_optim}
\end{equation}
Here, $\pi$ denotes a path from $(x,y)$ to $(0,0)$ and $\Pi$ denotes the set of all paths from $(x,y)$ to $(0,0)$. $|\pi|$ denotes the path length. $l^\pi_i(t)$ denotes the link state (at time $t$) of a link in path $\pi$ after $i$ steps. $\b l(0)$ denotes the state of all the links in the network at $t=0$.
Firstly, we need a way to order paths according to desirability. 


% \begin{definition}[Ordering of paths] For any two paths $\pi$ and $\pi'$, we say that $\pi \geq \pi'$ if the probability of reaching the destination is greater for path $\pi$ than $\pi'$. In other words, $\pi \geq \pi'$ when
% \begin{equation*}
%     \prod_{i=0}^{|\pi|-1} \P(l^\pi_i(t_c + i) = 1 | \b{l}(0)) \geq \prod_{i=0}^{|\pi'|-1} \P(l^{\pi'}_i(t_c + i) = 1 | \b{l}(0)).
% \end{equation*}
% \end{definition}

This optimization problem \eqref{eqn:centralized_scenarioA_optim} is non-trivial to solve. 
Since we are dealing with links having \textit{positive memory}, we are intuitively inclined to hope that choosing connected paths at $t=0$ would give us the best probability of reaching the destination, as these paths are likely to be ON as we traverse the route as well. 
We show that this intuition is true for a special case -- when there is a connected path $\pi$ at $t=0$ that is also one of the shortest paths from the source to the destination, it is a solution of \eqref{eqn:centralized_scenarioA_optim}.

\begin{lemma}\label{lemma:connected_path_length} For two paths $\pi$ and $\pi'$ that are connected at $t = 0$, $\pi \geq \pi'$ if and only if $|\pi| \leq |\pi'|$.
\end{lemma}
\begin{proof}
    \input{lemma1_proof}
\end{proof}

Using Lemma 
% The probability of the packet reaching the destination satellite, $P_{central}$, is given by
% \begin{align}
%     P_{central} = \P(\text{Path exists at }t = 0) \times \prod_{i=0}^{d}p_{11}(t_c + i),
% \end{align}
% where $d$ is the number of hops of the path 

\subsection{Optimal Centralized Policy In Scenario A}\label{sec:distributed_optimality_scenB}
